Robust decision-making under risk and ambiguity

Economists often estimate economic models on data and use the point estimates as a stand-in for the truth when studying the model's implications for optimal decision-making. This practice ignores model ambiguity, exposes the decision problem to misspecification, and ultimately leads to post-decision disappointment. Using statistical decision theory, we develop a framework to explore, evaluate, and optimize robust decision rules that explicitly account for estimation uncertainty. We show how to operationalize our analysis by studying robust decisions in a stochastic dynamic investment model in which a decision-maker directly accounts for uncertainty in the model's transition dynamics.

==> material/fig-decision-making.tex <==
% Decision-making with models across domains


\begin{tikzpicture}
   \fill[even odd rule, mediumblue!20, draw=mediumblue!30] circle (3.5);
   \fill[even odd rule, mediumblue] circle (1.7);

   \node at (0,0) [
      color = white,
      align = center
   ]{
      Decision-making\\
      with models
   };
   \arcarrow{ 85}{  -25}{ Robust Optimization  }
   \arcarrow{210}{95}{ Decision Theory }
   \arcarrow{215}{330}{ Economics  }
\end{tikzpicture}

==> material/fig_ambiguity_set.tex <==
\begin{tikzpicture}

% Circle circle
\node[circle, minimum size=5cm, draw] (circle small) {};
% without outlined border
%\node[circle, minimum size = 7.5cm, fill=tabblue!15] (circle large) {};
%\node[circle, minimum size=4.5cm, fill=tabblue] (circle small) {};

% Origin
\node[circle, draw, inner sep=1.5pt, fill=black, label=above:$\hat{p}$](origin) {};

% Alternative probability distributions
\node [fill=black, shape=circle, inner sep=1.5pt, label=below:$p_0$] (prob distribution eta low) at (-0.7,1.5) {};

% Lines
\draw[dashed, line width = 1.25pt] (origin) -- (10:2.5) node[midway, above]{$\rho$};

% Sets
\node[align=center, text width=6cm] at (0,-0.6) {\footnotesize $\{ p: D_{KL}(p  || \hat{p}) \leq  \rho \}$};

\end{tikzpicture}

%$\{\mathcal{P}: R(\mathcal{P} || \mathcal{P}_0) \leq \eta_{\text{high}} \}$


%\begin{tikzpicture}
%
%% Larger circle
%\node[circle, minimum size = 8cm, draw, fill=tabblue!15] (circle large) {};
%% Smaller circle
%\node[circle, minimum size=5cm, draw, fill=tabblue] (circle small) {};
%% without outlined border
%%\node[circle, minimum size = 7.5cm, fill=tabblue!15] (circle large) {};
%%\node[circle, minimum size=4.5cm, fill=tabblue] (circle small) {};
%
%% Origin
%\node[circle, draw, inner sep=1.5pt, fill=black, label=below:$\mathcal{P}_0$](origin) {};
%
%% Alternative probability distributions
%\node [fill=black, shape=circle, inner sep=1.5pt, label=below:$\tilde{\mathcal{P}}_{\eta_{\text{high}}}$] (prob distribution eta high) at (2.5,2.2) {};
%\node [fill=black, shape=circle, inner sep=1.5pt, label=below:$\tilde{\mathcal{P}}_{\eta_{\text{low}}}$] (prob distribution eta low) at (-0.7,1.5) {};
%
%% Lines
%\draw[dashed, line width = 1.25pt] (origin) -- (-190:4) node[above, xshift = 0.8cm, yshift = -0.2cm]{$\eta_{\text{high}}$};
%\draw[dashed, line width = 1.25pt] (origin) -- (10:2.5) node[midway, above]{$\eta_{\text{low}}$};
%
%% Sets
%\node[align=center	, text width=6cm] at (0,-3) {\small $\{ \mathcal{P}: R(\mathcal{P} || \mathcal{P}_0) \leq  \eta_{\text{high}} \}$};
%\node[align=center	, text width=6cm] at (0,-1.1) {\small $\{ \mathcal{P}: R(\mathcal{P} || \mathcal{P}_0) \leq  \eta_{\text{low}} \}$};
%
%\end{tikzpicture}
%
%%$\{\mathcal{P}: R(\mathcal{P} || \mathcal{P}_0) \leq \eta_{\text{high}} \}$

